Partial Density of States Ligand Field Theory (PDOS-LFT): Recovering a LFT-Like Picture and Application to Photoproperties of Ruthenium(II) Polypyridine Complexes

Gas phase density-functional theory (DFT) and time-dependent DFT (TD-DFT) calculations are reported for a data base of 98 ruthenium(II) polypyridine complexes. Comparison with X-ray crystal geometries and with experimental absorption spectra measured in solution show an excellent linear correlation with the results of the gas phase calculations. Comparing this with the usual chemical understanding based upon ligand field theory (LFT) is complicated by the large number of molecular orbitals present and especially by the heavy mixing of the antibonding metal e*$_{g}$ orbitals with ligand orbitals. Nevertheless, we show that a deeper understanding can be obtained by a partial density-of-states (PDOS) analysis which allows us to extract approximate metal t$_{2g}$ and e*$_{g}$ and ligand \pi* orbital energies in a well-defined way, thus providing a PDOS analogue of LFT (PDOS-LFT). Not only do PDOS-LFT energies generate a spectrochemical series for the ligands, but orbital energy differences provide good estimates of TD-DFT absorption energies. Encouraged by this success, we use frontier-molecular-orbital-theory-like reasoning to construct a model which allows us in most, but not all, of the cases studied to use PDOS-LFT energies to provide a semiquantitative relationship between luminescence lifetimes at room temperature and liquid nitrogen temperature.

==> main_edited_for arxiv/tables/PDOS.tex <==
% =======================================
% file: PDOS.tex
% last updated: 22 January 2017
% =======================================

\begin{table}
\caption{B3LYP PDOS.  An asterisk indicates that the $e^*_g$ orbitals are unbound
        (positive energy).
         \label{tab:PDOS_1}}
\begin{tabular}{ccc}
\hline \hline
number      & 6-31G       & 6-31G(d)       \\
\hline
({\bf 1})*  & Q4.8        & Q4.8           \\
({\bf 2})   &             &                \\
({\bf 3})*  & Q4.3        & Q4.3           \\
({\bf 4})   &             &                \\
({\bf 5})*  & Q4.10       & Q4.10          \\
({\bf 6})   &             &                \\
({\bf 7})*  & Q4.11       & Q4.11          \\
({\bf 8})   &             &                \\
({\bf 9})   &             &                \\
({\bf 10})  &             &                \\
({\bf 11})  &             &                \\
({\bf 12})  &             &                \\
({\bf 13})  &             &                \\
({\bf 14})  & Q4.15       & Q4.15          \\
({\bf 15})  & Q4.12       & Q4.12          \\
({\bf 16})  & Q4.13       & Q4.13          \\
({\bf 17})  & Q4.14       & Q4.14          \\
({\bf 18})  &             &                \\
({\bf 19})  &             &                \\
({\bf 20})  & Q4.16       & Q4.16          \\
({\bf 21})  & Q6.16       & Q6.16          \\
({\bf 22})  &             &                \\
({\bf 23})  & Q6.17       & Q6.17          \\
({\bf 24})  & Q6.18       & Q6.18          \\
({\bf 25})  & Q6.19       & Q6.19          \\
({\bf 26})  & Q6.20       & Q6.20          \\
({\bf 27})  & Q6.21       & Q6.21          \\
({\bf 28})  & Q6.22       & Q6.22          \\
({\bf 29})  & Q4.5        & Q4.5           \\
({\bf 30})  & Q4.2        & Q4.2           \\
({\bf 31})  & Q4.7        & Q4.7           \\
({\bf 32})  & Q4.9        & Q4.9           \\
({\bf 33})  &             &                \\
({\bf 34})  & Q6.31       & Q6.31          \\
({\bf 35})  & Q6.32       & Q6.32          \\
\hline \hline                                                 
\end{tabular}
\end{table}

% ----------------------------------------------------------------

\begin{table}
\caption{B3LYP PDOS. An asterisk indicates that the $e^*_g$ orbitals are unbound
        (positive energy).
         \label{tab:PDOS_2}}
\begin{tabular}{ccc}
\hline \hline
number       & 6-31G & 6-31G(d) \\
\hline
({\bf 36})  & Q6.33       & Q6.33          \\
({\bf 37})  & Q6.34       & Q6.34          \\
({\bf 38})  &             &                \\
({\bf 39})  &             &                \\
({\bf 40})  & Q6.35       & Q6.35          \\
({\bf 41})  & Q6.36       & Q6.36          \\
({\bf 42})  & Q6.37       & Q6.37          \\
({\bf 43})  &             &                \\
({\bf 44})  &             &                \\
({\bf 45})  &             &                \\
({\bf 46})  & Q6.38       & Q6.38          \\
({\bf 47})  & Q6.39       & Q6.39          \\
({\bf 48})  & Q6.40       & Q6.40          \\
({\bf 49})  &             &                \\
({\bf 50})  & Q6.41       & Q6.41          \\
({\bf 51})  &             &                \\
({\bf 52})  & Q6.23       & Q6.23          \\
({\bf 53})  & Q6.24       & Q6.24          \\
({\bf 54})  &             &                \\
({\bf 55})  & Q6.25       & Q6.25          \\
({\bf 56})  & Q6.26       & Q6.26          \\
({\bf 57})  & Q6.27       & Q6.27          \\
({\bf 58})  & Q6.28       & Q6.28          \\
({\bf 59})  &             &                \\
({\bf 60})  & Q6.29       & Q6.29          \\
({\bf 61})  & Q6.30       & Q6.30          \\
({\bf 62})  &             &                \\
({\bf 63})  &             &                \\
({\bf 64})* & Q6.2        & Q6.2           \\
({\bf 65})  &             &                \\
({\bf 66})* & Q6.3        & Q6.3           \\
({\bf 67})* & Q6.4        & Q6.4           \\
({\bf 68})* & Q6.5        & Q6.5           \\
({\bf 69})  &             &                \\
({\bf 70})  & Q6.6        & Q6.6           \\
\hline \hline                                                 
\end{tabular}
\end{table}

% ----------------------------------------------------------------

\begin{table}
\caption{B3LYP PDOS. An asterisk indicates that the $e^*_g$ orbitals are unbound
        (positive energy).
         \label{tab:PDOS_3}}
\begin{tabular}{ccc}
\hline \hline
number       & 6-31G & 6-31G(d) \\
\hline
({\bf 71})   & Q6.7         & Q6.7           \\
({\bf 72})   &              &                \\
({\bf 73})   & Q6.8         &                \\
({\bf 74})   & Q6.9         &                \\
({\bf 75})   & Q6.10        & Q6.10          \\
({\bf 76})   & Q6.11        & Q6.11          \\
({\bf 77})   & Q6.12        & Q6.12          \\
({\bf 78})   & Q6.1         & Q6.1           \\
({\bf 79})   & Q5.2         & Q5.2           \\
({\bf 80})   & Q5.3         & Q5.3           \\
({\bf 81})   & Q5.4         & Q5.4           \\
({\bf 82})   & Q5.5         & Q5.5           \\
({\bf 83})   & Q5.6         & Q5.6           \\
({\bf 84})   & Q5.7         & Q5.7           \\
({\bf 85})   & Q5.8         & Q5.8           \\
({\bf 86})   & Q5.9         &                \\
({\bf 87})   & Q5.10        & Q5.10          \\
({\bf 88})*  & Q6.13        & Q6.13          \\
({\bf 89})   & Q5.11        & Q5.11          \\
({\bf 90})   & Q6.14        & Q6.14          \\
({\bf 91})   & Q5.12        & Q5.12          \\
({\bf 92})   & Q5.13        & Q5.13          \\
({\bf 93})   & Q5.14        & Q5.14          \\
({\bf 94})   & Q5.15        & Q5.15          \\
({\bf 95})   & Q5.16        & Q5.16          \\
({\bf 96})   & Q5.17        & Q5.17          \\
({\bf 97})   & Q5.18        & Q5.18          \\
({\bf 98})   &              &                \\
({\bf 99})*  & Q4.4         & Q4.4           \\
({\bf 100})  & Q5.20        &                \\
({\bf 101})  & Q5.21        &                \\
({\bf 102})  &              &                \\
({\bf 103})* & Q4.6         & Q4.6           \\
({\bf 104})  & Q5.23, Q6.15 & Q6.15          \\
({\bf 105})  &              &                \\
\hline \hline                                                 
\end{tabular}
\end{table}

% ----------------------------------------------------------------

\begin{table}
\caption{B3LYP PDOS. An asterisk indicates that the $e^*_g$ orbitals are unbound
        (positive energy).
         \label{tab:PDOS_4}}
\begin{tabular}{ccc}
\hline \hline
number       & 6-31G      &    6-31G(d) \\
\hline
({\bf 106})* & Q4.1        & Q4.1           \\
({\bf 107})  & Q5.25       & Q5.25          \\
({\bf 108})  &             &                \\
({\bf 109})  & Q5.26       & Q5.26          \\
({\bf 110})  & Q5.27       &                \\
({\bf 111})* & Q5.28       & Q5.28          \\
\hline \hline                                                 
\end{tabular}
\end{table}

%%%%%
% EOF
%%%%%


==> main_edited_for arxiv/tables/spectra.tex <==
% =======================================
% file: spectra.tex
% last updated: 11 April 2017
% =======================================

\begin{table}
\caption{TD-B3LYP and experimental absorption spectra.
         \label{tab:spectra_1}}
\begin{tabular}{cccc}
\hline \hline
number      & 6-31G        & 6-31G(d)       & Expt.     \\
\hline
({\bf 1})   & Q4.7         & Q4.7           & Ref.~\cite{BCI+86} \\
({\bf 2})   & Q2.3         & Q2.3           & Ref.~\cite{GCS10} \\
({\bf 3})   & Q2.4         & Q2.4           & Ref.~\cite{FLH07} \\
({\bf 4})   & Q2.5, Q4.8   & Q2.5, Q4.8     &           \\
({\bf 5})   & Q2.2         & Q2.2           &           \\
({\bf 6})   & Q3.1         & Q3.1           &           \\
({\bf 7})   & Q2.6, Q4.9   & Q2.6, Q4.9     & Ref.~\cite{JFV+82} \\
({\bf 8})   &              &                &           \\
({\bf 9})   & Q2.5         & Q2.5           &           \\
({\bf 10})  &              &                &           \\
({\bf 11})  &              &                &           \\
({\bf 12})  &              &                &           \\
({\bf 13})  &              &                &           \\
({\bf 14})  & Q4.13        & Q4.13          & Ref.~\cite{SAF+78} \\
({\bf 15})  & Q4.10        & Q4.10          & Ref.~\cite{RAMC83} \\
({\bf 16})  & Q2.7, Q4.12  & Q2.7, Q4.12    &           \\
({\bf 17})  & Q2.8, Q4.11  & Q2.8, Q4.11    &           \\
({\bf 18})  & Q4.16        & Q4.16          &           \\
({\bf 19})  & Q5.1         & Q5.1           & Ref.~\cite{GBW78} \\
({\bf 20})  & Q4.14        & Q4.14          & Ref.~missing \\
({\bf 21})  & Q6.12        & Q6.12          &           \\
({\bf 22})  & Q2.9         & Q2.9           & Ref.~\cite{WJWR95,HXA+10} \\
({\bf 23})  & Q6.13        & Q6.13          & Ref.~\cite{JBB+86} \\
({\bf 24})  & Q2.10, Q6.14 & Q2.10, Q6.14   & Ref.~\cite{BGS+13} \\
({\bf 25})  & Q6.15        & Q6.15          & Ref.~\cite{K77} \\
({\bf 26})  & Q2.11, Q6.16 & Q2.11, Q6.16   &           \\
({\bf 27})  & Q6.17        & Q6.17          & Ref.~\cite{DKSS03} \\
({\bf 28})  & Q6.18        & Q6.18          &           \\
({\bf 29})  & Q4.4         & Q4.4           & Ref.~\cite{M83} \\
({\bf 30})  & Q4.2         & Q4.2           & Ref.~\cite{M83} \\
({\bf 31})  & Q2.12, Q4.6  & Q2.12, Q4.6    & Ref.~\cite{EL78} \\
({\bf 32})  & Q2.13        & Q2.13          & Ref.~\cite{LNZ+13} \\
({\bf 33})  &              &                &           \\
({\bf 34})  & Q6.27        & Q6.27          & Ref.~\cite{BJB+84} \\ 
({\bf 35})  & Q6.28        & Q6.28          & Ref.~\cite{BJB+84} \\
\hline \hline                                                 
\end{tabular}
\end{table}

% ----------------------------------------------------------------

\begin{table}
\caption{TD-B3LYP and experimental absorption spectra.
         \label{tab:spectra_2}}
\begin{tabular}{cccc}
\hline \hline
number       & 6-31G & 6-31G(d) & Expt.    \\
\hline
({\bf 36})  & Q2.14       & Q2.14          & Ref.~\cite{TVD+87} \\
({\bf 37})  & Q6.29       & Q6.29          & Ref.~\cite{JBBV81} \\
({\bf 38})  & Q6.30       & Q6.30          & Ref.~\cite{BJB+84} \\
({\bf 39})  & Q6.31       & Q6.31          & Ref.~\cite{JFV+82} \\
({\bf 40})  & Q6.32       & Q6.32          & Ref.~\cite{JBB+86} \\
({\bf 41})  & Q6.33       & Q6.33          &           \\
({\bf 42})  & Q6.34       & Q6.34          &           \\
({\bf 43})  &             &                &           \\
({\bf 44})  &             &                &           \\
({\bf 45})  &             &                &           \\
({\bf 46})  & Q6.35       & Q6.35          & Ref.~\cite{JBBV81} \\
({\bf 47})  & Q6.36       & Q6.36          & Ref.~\cite{BJB+84} \\
({\bf 48})  & Q2.15       & Q2.15          & Ref.~\cite{CDH+09} \\
({\bf 49})  &             &                &           \\
({\bf 50})  & Q6.37       & Q6.37          & Ref.~\cite{K77} \\
({\bf 51})  &             &                &           \\
({\bf 52})  & Q6.19       & Q6.19          & Ref.~\cite{JBB+86} \\
({\bf 53})  & Q6.20       & Q6.20          & Ref.~\cite{K77} \\
({\bf 54})  &             &                &           \\
({\bf 55})  & Q6.21       & Q6.21          & Ref.~\cite{K77} \\
({\bf 56})  & Q6.22       & Q6.22          & Ref.~\cite{K77} \\
({\bf 57})  & Q6.23       & Q6.23          & Ref.~\cite{K77} \\
({\bf 58})  & Q6.24       & Q6.24          & Ref.~\cite{K77} \\
({\bf 59})  &             &                &           \\
({\bf 60})  & Q6.25       & Q6.25          & Ref.~\cite{KBW94} \\
({\bf 61})  &             &                &           \\
({\bf 62})  &             &                &           \\
({\bf 63})  & Q2.17       & Q2.17          & Ref.~\cite{YMK+04} \\
({\bf 64})  & Q2.16, Q6.1 & Q2.16, Q6.1    & Ref.~\cite{CAY+12} \\
({\bf 65})  &             &                &           \\
({\bf 66})  & Q2.18       & Q2.18          & Ref.~\cite{FKS80,SML+13} \\
({\bf 67})  & Q6.2        & Q6.2           & Ref.~\cite{N82} \\
({\bf 68})  &             &                &           \\
({\bf 69})  & Q6.4        & Q6.4           & Ref.~\cite{N82} \\
({\bf 70})  & Q6.5        & Q6.5           & Ref.~\cite{MMIC03} \\
\hline \hline                                                 
\end{tabular}
\end{table}

% ----------------------------------------------------------------

\begin{table}
\caption{TD-B3LYP and experimental absorption spectra.
         \label{tab:spectra_3}}
\begin{tabular}{cccc}
\hline \hline
number       & 6-31G & 6-31G(d) & Expt.    \\
\hline
({\bf 71})  & Q6.6        & Q6.6           & Ref.~\cite{GBW78} \\
({\bf 72})  &             &                &           \\
({\bf 73})  & Q6.7        & Q6.7           & Ref.~\cite{BM88} \\
({\bf 74})  & Q3.2        & Q3.2           & Ref.~\cite{SSG+08} \\
({\bf 75})  & Q6.8        & Q6.8           & Ref.~\cite{FKS80} \\
({\bf 76})  & Q6.9        & Q6.9           & Ref.~\cite{BJB+84} \\
({\bf 77})  & Q3.3        & Q3.3           & Ref.~\cite{LRE+04} \\
({\bf 78})  & Q5.2        & Q5.2           & Ref.~\cite{BJB+84} \\
({\bf 79})  &             &                &           \\
({\bf 80})  & Q5.3        & Q5.3           & Ref.~\cite{BJB+84}  \\
({\bf 81})  & Q5.4        & Q5.4           & Ref.~\cite{BJB+84,WHH+12b} \\
({\bf 82})  & Q5.5        & Q5.5           & Ref.~\cite{K82} \\
({\bf 83})  & Q5.6        & Q5.6           & Ref.~\cite{K82,WHH+12b} \\
({\bf 84})  & Q5.7        & Q5.7           & Ref.~\cite{FKS80} \\
({\bf 85})  & Q5.8        & Q5.8           & Ref.~\cite{FKS80} \\
({\bf 86})  & Q5.9        & Q5.9           & Ref.~\cite{LBC+76} \\
({\bf 87})  & Q5.10       & Q5.10          & Ref.~\cite{GBW78} \\
({\bf 88})  & Q6.11       & Q6.11          & Ref.~\cite{SD82} \\
({\bf 89})  & Q5.11       & Q5.11          &           \\
({\bf 90})  & Q6.10       & Q6.10          & Ref.~\cite{SD82} \\
({\bf 91})  & Q3.4        & Q3.4           & Ref.~\cite{DSH+03} \\
({\bf 92})  & Q5.12       & Q5.12          & Ref.~\cite{KK84} \\
({\bf 93})  & Q5.13       & Q5.13          & Ref.~\cite{BJB+84} \\
({\bf 94})  & Q5.14       & Q5.14          & Ref.~\cite{OHD84} \\
({\bf 95})  & Q5.15       & Q5.15          & Ref.~\cite{K82} \\
({\bf 96})  & Q5.16       & Q5.16          & Ref.~\cite{K82} \\
({\bf 97})  & Q5.17       & Q5.17          & Ref.~\cite{ASWK84} \\
({\bf 98})  & Q5.18       & Q5.18          & Ref.~\cite{BJB+83} \\
({\bf 99})  & Q4.3        & Q4.3           & Ref.~\cite{JBB+88} \\
({\bf 100}) & Q5.19       & Q5.19          & Ref.~\cite{JBBV81} \\
({\bf 101}) & Q5.20       & Q5.20          & Ref.~\cite{ASWK84} \\
({\bf 102}) & Q5.21       & Q5.21          & Ref.~\cite{BJB+83} \\
({\bf 103}) & Q4.5        & Q4.5           & Ref.~\cite{JBB+88} \\
({\bf 104}) &             &                &           \\
({\bf 105}) & Q5.22       & Q5.22          & Ref.~\cite{BJB+83} \\
\hline \hline                                                 
\end{tabular}
\end{table}

% ----------------------------------------------------------------

\begin{table}
\caption{TD-B3LYP and experimental absorption spectra.
         \label{tab:spectra_4}}
\begin{tabular}{cccc}
\hline \hline
number       & 6-31G      &    6-31G(d) & Expt.    \\
\hline
({\bf 106}) & Q4.1        & Q4.1           & Refs.~\cite{JBB+88} \\
({\bf 107}) & Q5.23       & Q5.23          & Refs.~\cite{BVJ+82} \\
({\bf 108}) & Q2.1        & Q2.1           & Refs.~\cite{HVD12,SCC+94,JCD+09} \\
({\bf 109}) & Q5.24       & Q5.24          & Refs.~\cite{SC81} \\
({\bf 110}) & Q5.25       & Q5.25          & Refs.~\cite{SC81} \\
({\bf 111}) & Q5.26       & Q5.26          & Refs.~\cite{SC81} \\
\hline \hline                                                 
\end{tabular}
\end{table}

%%%%%
% EOF
%%%%%


==> tables/PDOS.tex <==
% =======================================
% file: PDOS.tex
% last updated: 22 January 2017
% =======================================

\begin{table}
\caption{B3LYP PDOS.  An asterisk indicates that the $e^*_g$ orbitals are unbound
        (positive energy).
         \label{tab:PDOS_1}}
\begin{tabular}{ccc}
\hline \hline
number      & 6-31G       & 6-31G(d)       \\
\hline
({\bf 1})*  & Q4.8        & Q4.8           \\
({\bf 2})   &             &                \\
({\bf 3})*  & Q4.3        & Q4.3           \\
({\bf 4})   &             &                \\
({\bf 5})*  & Q4.10       & Q4.10          \\
({\bf 6})   &             &                \\
({\bf 7})*  & Q4.11       & Q4.11          \\
({\bf 8})   &             &                \\
({\bf 9})   &             &                \\
({\bf 10})  &             &                \\
({\bf 11})  &             &                \\
({\bf 12})  &             &                \\
({\bf 13})  &             &                \\
({\bf 14})  & Q4.15       & Q4.15          \\
({\bf 15})  & Q4.12       & Q4.12          \\
({\bf 16})  & Q4.13       & Q4.13          \\
({\bf 17})  & Q4.14       & Q4.14          \\
({\bf 18})  &             &                \\
({\bf 19})  &             &                \\
({\bf 20})  & Q4.16       & Q4.16          \\
({\bf 21})  & Q6.16       & Q6.16          \\
({\bf 22})  &             &                \\
({\bf 23})  & Q6.17       & Q6.17          \\
({\bf 24})  & Q6.18       & Q6.18          \\
({\bf 25})  & Q6.19       & Q6.19          \\
({\bf 26})  & Q6.20       & Q6.20          \\
({\bf 27})  & Q6.21       & Q6.21          \\
({\bf 28})  & Q6.22       & Q6.22          \\
({\bf 29})  & Q4.5        & Q4.5           \\
({\bf 30})  & Q4.2        & Q4.2           \\
({\bf 31})  & Q4.7        & Q4.7           \\
({\bf 32})  & Q4.9        & Q4.9           \\
({\bf 33})  &             &                \\
({\bf 34})  & Q6.31       & Q6.31          \\
({\bf 35})  & Q6.32       & Q6.32          \\
\hline \hline                                                 
\end{tabular}
\end{table}

% ----------------------------------------------------------------

\begin{table}
\caption{B3LYP PDOS. An asterisk indicates that the $e^*_g$ orbitals are unbound
        (positive energy).
         \label{tab:PDOS_2}}
\begin{tabular}{ccc}
\hline \hline
number       & 6-31G & 6-31G(d) \\
\hline
({\bf 36})  & Q6.33       & Q6.33          \\
({\bf 37})  & Q6.34       & Q6.34          \\
({\bf 38})  &             &                \\
({\bf 39})  &             &                \\
({\bf 40})  & Q6.35       & Q6.35          \\
({\bf 41})  & Q6.36       & Q6.36          \\
({\bf 42})  & Q6.37       & Q6.37          \\
({\bf 43})  &             &                \\
({\bf 44})  &             &                \\
({\bf 45})  &             &                \\
({\bf 46})  & Q6.38       & Q6.38          \\
({\bf 47})  & Q6.39       & Q6.39          \\
({\bf 48})  & Q6.40       & Q6.40          \\
({\bf 49})  &             &                \\
({\bf 50})  & Q6.41       & Q6.41          \\
({\bf 51})  &             &                \\
({\bf 52})  & Q6.23       & Q6.23          \\
({\bf 53})  & Q6.24       & Q6.24          \\
({\bf 54})  &             &                \\
({\bf 55})  & Q6.25       & Q6.25          \\
({\bf 56})  & Q6.26       & Q6.26          \\
({\bf 57})  & Q6.27       & Q6.27          \\
({\bf 58})  & Q6.28       & Q6.28          \\
({\bf 59})  &             &                \\
({\bf 60})  & Q6.29       & Q6.29          \\
({\bf 61})  & Q6.30       & Q6.30          \\
({\bf 62})  &             &                \\
({\bf 63})  &             &                \\
({\bf 64})* & Q6.2        & Q6.2           \\
({\bf 65})  &             &                \\
({\bf 66})* & Q6.3        & Q6.3           \\
({\bf 67})* & Q6.4        & Q6.4           \\
({\bf 68})* & Q6.5        & Q6.5           \\
({\bf 69})  &             &                \\
({\bf 70})  & Q6.6        & Q6.6           \\
\hline \hline                                                 
\end{tabular}
\end{table}

% ----------------------------------------------------------------

\begin{table}
\caption{B3LYP PDOS. An asterisk indicates that the $e^*_g$ orbitals are unbound
        (positive energy).
         \label{tab:PDOS_3}}
\begin{tabular}{ccc}
\hline \hline
number       & 6-31G & 6-31G(d) \\
\hline
({\bf 71})   & Q6.7         & Q6.7           \\
({\bf 72})   &              &                \\
({\bf 73})   & Q6.8         &                \\
({\bf 74})   & Q6.9         &                \\
({\bf 75})   & Q6.10        & Q6.10          \\
({\bf 76})   & Q6.11        & Q6.11          \\
({\bf 77})   & Q6.12        & Q6.12          \\
({\bf 78})   & Q6.1         & Q6.1           \\
({\bf 79})   & Q5.2         & Q5.2           \\
({\bf 80})   & Q5.3         & Q5.3           \\
({\bf 81})   & Q5.4         & Q5.4           \\
({\bf 82})   & Q5.5         & Q5.5           \\
({\bf 83})   & Q5.6         & Q5.6           \\
({\bf 84})   & Q5.7         & Q5.7           \\
({\bf 85})   & Q5.8         & Q5.8           \\
({\bf 86})   & Q5.9         &                \\
({\bf 87})   & Q5.10        & Q5.10          \\
({\bf 88})*  & Q6.13        & Q6.13          \\
({\bf 89})   & Q5.11        & Q5.11          \\
({\bf 90})   & Q6.14        & Q6.14          \\
({\bf 91})   & Q5.12        & Q5.12          \\
({\bf 92})   & Q5.13        & Q5.13          \\
({\bf 93})   & Q5.14        & Q5.14          \\
({\bf 94})   & Q5.15        & Q5.15          \\
({\bf 95})   & Q5.16        & Q5.16          \\
({\bf 96})   & Q5.17        & Q5.17          \\
({\bf 97})   & Q5.18        & Q5.18          \\
({\bf 98})   &              &                \\
({\bf 99})*  & Q4.4         & Q4.4           \\
({\bf 100})  & Q5.20        &                \\
({\bf 101})  & Q5.21        &                \\
({\bf 102})  &              &                \\
({\bf 103})* & Q4.6         & Q4.6           \\
({\bf 104})  & Q5.23, Q6.15 & Q6.15          \\
({\bf 105})  &              &                \\
\hline \hline                                                 
\end{tabular}
\end{table}

% ----------------------------------------------------------------

\begin{table}
\caption{B3LYP PDOS. An asterisk indicates that the $e^*_g$ orbitals are unbound
        (positive energy).
         \label{tab:PDOS_4}}
\begin{tabular}{ccc}
\hline \hline
number       & 6-31G      &    6-31G(d) \\
\hline
({\bf 106})* & Q4.1        & Q4.1           \\
({\bf 107})  & Q5.25       & Q5.25          \\
({\bf 108})  &             &                \\
({\bf 109})  & Q5.26       & Q5.26          \\
({\bf 110})  & Q5.27       &                \\
({\bf 111})* & Q5.28       & Q5.28          \\
\hline \hline                                                 
\end{tabular}
\end{table}

%%%%%
% EOF
%%%%%


==> tables/spectra.tex <==
% =======================================
% file: spectra.tex
% last updated: 11 April 2017
% =======================================

\begin{table}
\caption{TD-B3LYP and experimental absorption spectra.
         \label{tab:spectra_1}}
\begin{tabular}{cccc}
\hline \hline
number      & 6-31G        & 6-31G(d)       & Expt.     \\
\hline
({\bf 1})   & Q4.7         & Q4.7           & Ref.~\cite{BCI+86} \\
({\bf 2})   & Q2.3         & Q2.3           & Ref.~\cite{GCS10} \\
({\bf 3})   & Q2.4         & Q2.4           & Ref.~\cite{FLH07} \\
({\bf 4})   & Q2.5, Q4.8   & Q2.5, Q4.8     &           \\
({\bf 5})   & Q2.2         & Q2.2           &           \\
({\bf 6})   & Q3.1         & Q3.1           &           \\
({\bf 7})   & Q2.6, Q4.9   & Q2.6, Q4.9     & Ref.~\cite{JFV+82} \\
({\bf 8})   &              &                &           \\
({\bf 9})   & Q2.5         & Q2.5           &           \\
({\bf 10})  &              &                &           \\
({\bf 11})  &              &                &           \\
({\bf 12})  &              &                &           \\
({\bf 13})  &              &                &           \\
({\bf 14})  & Q4.13        & Q4.13          & Ref.~\cite{SAF+78} \\
({\bf 15})  & Q4.10        & Q4.10          & Ref.~\cite{RAMC83} \\
({\bf 16})  & Q2.7, Q4.12  & Q2.7, Q4.12    &           \\
({\bf 17})  & Q2.8, Q4.11  & Q2.8, Q4.11    &           \\
({\bf 18})  & Q4.16        & Q4.16          &           \\
({\bf 19})  & Q5.1         & Q5.1           & Ref.~\cite{GBW78} \\
({\bf 20})  & Q4.14        & Q4.14          & Ref.~missing \\
({\bf 21})  & Q6.12        & Q6.12          &           \\
({\bf 22})  & Q2.9         & Q2.9           & Ref.~\cite{WJWR95,HXA+10} \\
({\bf 23})  & Q6.13        & Q6.13          & Ref.~\cite{JBB+86} \\
({\bf 24})  & Q2.10, Q6.14 & Q2.10, Q6.14   & Ref.~\cite{BGS+13} \\
({\bf 25})  & Q6.15        & Q6.15          & Ref.~\cite{K77} \\
({\bf 26})  & Q2.11, Q6.16 & Q2.11, Q6.16   &           \\
({\bf 27})  & Q6.17        & Q6.17          & Ref.~\cite{DKSS03} \\
({\bf 28})  & Q6.18        & Q6.18          &           \\
({\bf 29})  & Q4.4         & Q4.4           & Ref.~\cite{M83} \\
({\bf 30})  & Q4.2         & Q4.2           & Ref.~\cite{M83} \\
({\bf 31})  & Q2.12, Q4.6  & Q2.12, Q4.6    & Ref.~\cite{EL78} \\
({\bf 32})  & Q2.13        & Q2.13          & Ref.~\cite{LNZ+13} \\
({\bf 33})  &              &                &           \\
({\bf 34})  & Q6.27        & Q6.27          & Ref.~\cite{BJB+84} \\ 
({\bf 35})  & Q6.28        & Q6.28          & Ref.~\cite{BJB+84} \\
\hline \hline                                                 
\end{tabular}
\end{table}

% ----------------------------------------------------------------

\begin{table}
\caption{TD-B3LYP and experimental absorption spectra.
         \label{tab:spectra_2}}
\begin{tabular}{cccc}
\hline \hline
number       & 6-31G & 6-31G(d) & Expt.    \\
\hline
({\bf 36})  & Q2.14       & Q2.14          & Ref.~\cite{TVD+87} \\
({\bf 37})  & Q6.29       & Q6.29          & Ref.~\cite{JBBV81} \\
({\bf 38})  & Q6.30       & Q6.30          & Ref.~\cite{BJB+84} \\
({\bf 39})  & Q6.31       & Q6.31          & Ref.~\cite{JFV+82} \\
({\bf 40})  & Q6.32       & Q6.32          & Ref.~\cite{JBB+86} \\
({\bf 41})  & Q6.33       & Q6.33          &           \\
({\bf 42})  & Q6.34       & Q6.34          &           \\
({\bf 43})  &             &                &           \\
({\bf 44})  &             &                &           \\
({\bf 45})  &             &                &           \\
({\bf 46})  & Q6.35       & Q6.35          & Ref.~\cite{JBBV81} \\
({\bf 47})  & Q6.36       & Q6.36          & Ref.~\cite{BJB+84} \\
({\bf 48})  & Q2.15       & Q2.15          & Ref.~\cite{CDH+09} \\
({\bf 49})  &             &                &           \\
({\bf 50})  & Q6.37       & Q6.37          & Ref.~\cite{K77} \\
({\bf 51})  &             &                &           \\
({\bf 52})  & Q6.19       & Q6.19          & Ref.~\cite{JBB+86} \\
({\bf 53})  & Q6.20       & Q6.20          & Ref.~\cite{K77} \\
({\bf 54})  &             &                &           \\
({\bf 55})  & Q6.21       & Q6.21          & Ref.~\cite{K77} \\
({\bf 56})  & Q6.22       & Q6.22          & Ref.~\cite{K77} \\
({\bf 57})  & Q6.23       & Q6.23          & Ref.~\cite{K77} \\
({\bf 58})  & Q6.24       & Q6.24          & Ref.~\cite{K77} \\
({\bf 59})  &             &                &           \\
({\bf 60})  & Q6.25       & Q6.25          & Ref.~\cite{KBW94} \\
({\bf 61})  &             &                &           \\
({\bf 62})  &             &                &           \\
({\bf 63})  & Q2.17       & Q2.17          & Ref.~\cite{YMK+04} \\
({\bf 64})  & Q2.16, Q6.1 & Q2.16, Q6.1    & Ref.~\cite{CAY+12} \\
({\bf 65})  &             &                &           \\
({\bf 66})  & Q2.18       & Q2.18          & Ref.~\cite{FKS80,SML+13} \\
({\bf 67})  & Q6.2        & Q6.2           & Ref.~\cite{N82} \\
({\bf 68})  &             &                &           \\
({\bf 69})  & Q6.4        & Q6.4           & Ref.~\cite{N82} \\
({\bf 70})  & Q6.5        & Q6.5           & Ref.~\cite{MMIC03} \\
\hline \hline                                                 
\end{tabular}
\end{table}

% ----------------------------------------------------------------

\begin{table}
\caption{TD-B3LYP and experimental absorption spectra.
         \label{tab:spectra_3}}
\begin{tabular}{cccc}
\hline \hline
number       & 6-31G & 6-31G(d) & Expt.    \\
\hline
({\bf 71})  & Q6.6        & Q6.6           & Ref.~\cite{GBW78} \\
({\bf 72})  &             &                &           \\
({\bf 73})  & Q6.7        & Q6.7           & Ref.~\cite{BM88} \\
({\bf 74})  & Q3.2        & Q3.2           & Ref.~\cite{SSG+08} \\
({\bf 75})  & Q6.8        & Q6.8           & Ref.~\cite{FKS80} \\
({\bf 76})  & Q6.9        & Q6.9           & Ref.~\cite{BJB+84} \\
({\bf 77})  & Q3.3        & Q3.3           & Ref.~\cite{LRE+04} \\
({\bf 78})  & Q5.2        & Q5.2           & Ref.~\cite{BJB+84} \\
({\bf 79})  &             &                &           \\
({\bf 80})  & Q5.3        & Q5.3           & Ref.~\cite{BJB+84}  \\
({\bf 81})  & Q5.4        & Q5.4           & Ref.~\cite{BJB+84,WHH+12b} \\
({\bf 82})  & Q5.5        & Q5.5           & Ref.~\cite{K82} \\
({\bf 83})  & Q5.6        & Q5.6           & Ref.~\cite{K82,WHH+12b} \\
({\bf 84})  & Q5.7        & Q5.7           & Ref.~\cite{FKS80} \\
({\bf 85})  & Q5.8        & Q5.8           & Ref.~\cite{FKS80} \\
({\bf 86})  & Q5.9        & Q5.9           & Ref.~\cite{LBC+76} \\
({\bf 87})  & Q5.10       & Q5.10          & Ref.~\cite{GBW78} \\
({\bf 88})  & Q6.11       & Q6.11          & Ref.~\cite{SD82} \\
({\bf 89})  & Q5.11       & Q5.11          &           \\
({\bf 90})  & Q6.10       & Q6.10          & Ref.~\cite{SD82} \\
({\bf 91})  & Q3.4        & Q3.4           & Ref.~\cite{DSH+03} \\
({\bf 92})  & Q5.12       & Q5.12          & Ref.~\cite{KK84} \\
({\bf 93})  & Q5.13       & Q5.13          & Ref.~\cite{BJB+84} \\
({\bf 94})  & Q5.14       & Q5.14          & Ref.~\cite{OHD84} \\
({\bf 95})  & Q5.15       & Q5.15          & Ref.~\cite{K82} \\
({\bf 96})  & Q5.16       & Q5.16          & Ref.~\cite{K82} \\
({\bf 97})  & Q5.17       & Q5.17          & Ref.~\cite{ASWK84} \\
({\bf 98})  & Q5.18       & Q5.18          & Ref.~\cite{BJB+83} \\
({\bf 99})  & Q4.3        & Q4.3           & Ref.~\cite{JBB+88} \\
({\bf 100}) & Q5.19       & Q5.19          & Ref.~\cite{JBBV81} \\
({\bf 101}) & Q5.20       & Q5.20          & Ref.~\cite{ASWK84} \\
({\bf 102}) & Q5.21       & Q5.21          & Ref.~\cite{BJB+83} \\
({\bf 103}) & Q4.5        & Q4.5           & Ref.~\cite{JBB+88} \\
({\bf 104}) &             &                &           \\
({\bf 105}) & Q5.22       & Q5.22          & Ref.~\cite{BJB+83} \\
\hline \hline                                                 
\end{tabular}
\end{table}

% ----------------------------------------------------------------

\begin{table}
\caption{TD-B3LYP and experimental absorption spectra.
         \label{tab:spectra_4}}
\begin{tabular}{cccc}
\hline \hline
number       & 6-31G      &    6-31G(d) & Expt.    \\
\hline
({\bf 106}) & Q4.1        & Q4.1           & Refs.~\cite{JBB+88} \\
({\bf 107}) & Q5.23       & Q5.23          & Refs.~\cite{BVJ+82} \\
({\bf 108}) & Q2.1        & Q2.1           & Refs.~\cite{HVD12,SCC+94,JCD+09} \\
({\bf 109}) & Q5.24       & Q5.24          & Refs.~\cite{SC81} \\
({\bf 110}) & Q5.25       & Q5.25          & Refs.~\cite{SC81} \\
({\bf 111}) & Q5.26       & Q5.26          & Refs.~\cite{SC81} \\
\hline \hline                                                 
\end{tabular}
\end{table}

%%%%%
% EOF
%%%%%

